Simultaneous Event Execution in Heterogeneous Wireless Sensor Networks

We present a synchronization algorithm to let nodes in a sensor network simultaneously execute a task at a given point in time. In contrast to other time synchronization algorithms we do not provide a global time basis that is shared on all nodes. Instead, any node in the network can spontaneously initiate a process that allows the simultaneous execution of arbitrary tasks. We show that our approach is beneficial in scenarios where a global time is not needed, as it requires little communication compared with other time synchronization algorithms. We also show that our algorithm works in heterogeneous systems where the hardware provides highly varying clock accuracy. Moreover, heterogeneity does not only affect the hardware, but also the communication channels. We deal with different connection types---from highly unreliable and fluctuating wireless channels to reliable and fast wired connections.

==> assumptions.tex <==
\begin{itemize}
\item propagation delay remains constant for dense networks
\item time between sending a packet in the MAC layer and calling the
  confirm method is equal on all nodes
\item clocks run at constant speed (i.e. constant temperature,
  constant supply voltage)
\end{itemize}

